What Makes a GitHub Issue Ready for Copilot?

AI-agents help developers in different coding tasks, such as developing new features, fixing bugs, and reviewing code. Developers can write a Github issue and assign it to an AI-agent like Copilot for implementation. Based on the issue and its related discussion, the AI-agent performs a plan for the implementation, and executes it. However, the performance of AI-agents and LLMs heavily depends on the input they receive. For instance, a GitHub issue that is unclear or not well scoped might not lead to a successful implementation that will eventually be merged. GitHub Copilot provides a set of best practice recommendations that are limited and high-level. In this paper, we build a set of 32 detailed criteria that we leverage to measure the quality of GitHub issues to make them suitable for AI-agents. We compare the GitHub issues that lead to a merged pull request versus closed pull request. Then, we build an interpretable machine learning model to predict the likelihood of a GitHub issue resulting in a merged pull request. We observe that pull requests that end up being merged are those originating from issues that are shorter, well scoped, with clear guidance and hints about the relevant artifacts for an issue, and with guidance on how to perform the implementation. Issues with external references including configuration, context setup, dependencies or external APIs are associated with lower merge rates. We built an interpretable machine learning model to help users identify how to improve a GitHub issue to increase the chances of the issue resulting in a merged pull request by Copilot. Our model has a median AUC of 72\%. Our results shed light on quality metrics relevant for writing GitHub issues and motivate future studies further investigate the writing of GitHub issues as a first-class software engineering activity in the era of AI-teammates.

==> sections/cover_letter.tex <==
\onecolumn   
\setcounter{section}{0}


The paper reports completely new research results and does not extend prior work. The contribution of this paper is a set of 32 criteria to evaluate the quality of GitHub issues to make them ready for AI-agents. These criteria are used to empirically compare issues based on their likelihood of ending with a merged pull request created by an AI-agent. We also built a novel machine learning model that predicts the likelihood of a GitHub issue ending with a merged pull request. We evaluate the quality of LLMs on quantifying the quality of a GitHub issue and the performances of our prediction model. 

